EdgeMixup: Improving Fairness for Skin Disease Classification and Segmentation

Skin lesions can be an early indicator of a wide range of infectious and other diseases. The use of deep learning (DL) models to diagnose skin lesions has great potential in assisting clinicians with prescreening patients. However, these models often learn biases inherent in training data, which can lead to a performance gap in the diagnosis of people with light and/or dark skin tones. To the best of our knowledge, limited work has been done on identifying, let alone reducing, model bias in skin disease classification and segmentation. In this paper, we examine DL fairness and demonstrate the existence of bias in classification and segmentation models for subpopulations with darker skin tones compared to individuals with lighter skin tones, for specific diseases including Lyme, Tinea Corporis and Herpes Zoster. Then, we propose a novel preprocessing, data alteration method, called EdgeMixup, to improve model fairness with a linear combination of an input skin lesion image and a corresponding a predicted edge detection mask combined with color saturation alteration. For the task of skin disease classification, EdgeMixup outperforms much more complex competing methods such as adversarial approaches, achieving a 10.99% reduction in accuracy gap between light and dark skin tone samples, and resulting in 8.4% improved performance for an underrepresented subpopulation.

==> sections/acknowledgments.tex <==
\section{Acknowledgments}
\label{sec:acknowledgments}

==> sections/metrics.tex <==
\section{Metrics}
\label{sec:metrics}

The fairness of both classification and segmentation models are evaluated using a series of joint utility functions that balance the performance of said models and the gap between subpopulations of the protected factor. This joint utility function was first introduced by~\cite{paul2020TARA} for the case of classification accuracy, expressed as follows:
\begin{equation}
CAI_{\alpha} = \alpha (acc_{gap}^b - acc_{gap}^d) + (1 - \alpha) (acc^d - acc^b).
\end{equation}
The $CAI_{\alpha}$ metric uses $\alpha$ to balance the importance of a reduction in the accuracy gap and an improvement in accuracy between the baseline $acc^b$ and debiased $acc^d$ methods. Where the accuracy gap of the baseline $acc_{gap}^b$ and debiased $acc_{gap}^d$ methods are computed as the difference between the accuracy of the subpopulations of $S$, which in this case is binary: light skin tone and dark skin tone. Moreover,~\cite{paul2020TARA} also introduced a variation of the fairness utility based on area under the curve $AUC$ metric, as illustrated below:
\begin{equation}
CAUCI_{\alpha} = \alpha (AUC_{gap}^b - AUC_{gap}^d) + (1 - \alpha) (AUC^d - AUC^b).
\end{equation}
$CAUCI_{\alpha}$ operates in a similar manner to $CAI_{\alpha}$ where AUC gap ($AUC_{gap}^b$ and $AUC_{gap}^d$) reduction importance is balanced with an increase in the change of AUC ($AUC^d$ - $AUC^b$) for the baseline $b$ and debiased $d$ methods. 
